How to "DODGE" Complex Software Analytics?

Machine learning techniques applied to software engineering tasks can be improved by hyperparameter optimization, i.e., automatic tools that find good settings for a learner's control parameters. We show that such hyperparameter optimization can be unnecessarily slow, particularly when the optimizers waste time exploring "redundant tunings"', i.e., pairs of tunings which lead to indistinguishable results. By ignoring redundant tunings, DODGE, a tuning tool, runs orders of magnitude faster, while also generating learners with more accurate predictions than seen in prior state-of-the-art approaches.

==> fft.tex <==
\begin{table}[!t]
\caption{FFTrees: an ensemble algorithm to   sample results space,
$M$  number of times.}\label{fig:dart}
\small \begin{tabular}{|p{.95\linewidth}|}\hline
INPUT: 
\bi
\item A dataset, such as one from \tbl{data};
\item A goal predicate $p$; e.g., ${P_{\mathit{opt}}}$ or  $\mathit{dis2Heaven}$;
\item $M,N$=  number of models, number of ranges used per model
\ei
OUTPUT:
\bi\item Score of the best model when applied to data not used for training.
\ei 
PROCEDURE:
\bi
\item Separate the data into train and test;
\item On the train data, build an ensemble and select the best:
\bi
\item   For $i=1$ to $M$  do
\be
\item Divide numeric attributes into ranges; 
\item Find $N$ {\em extreme} ranges  that score highest and lowest on $p$;  
\item  Combine some the extreme ranges into   model $i$;
\item Score $i$   using $p$;
\item Keep the best scoring model.
\ee
\ei
\item On the test data:
\bi
\item Return the $p$ score of  the best scoring model.
\ei
\ei 
NOTES:
\bi
\item
For training step (2), we use  {\em extreme} ranges in order to maximize the spread of the darts around the results space.
\item
To  keep this simple,  the  discretizer  used in   training step (1)  just divides the
numeric data on its median value.
\ei\\\hline
\end{tabular}

\end{table}

==> reply.tex <==
\newpage
  \pagenumbering{roman}
\setcounter{page}{1}

\newenvironment{com}{\color{blue}\begin{itshape}}{\end{itshape}\vspace{1ex}}

\section*{Response to Reviewers}

Please see our replies to reviewer comments, below. Note that anything in \begin{com}
blue
\end{com} is from the reviewers. Our replies are in  \textbf{black} text.

\subsection*{Associate Editor}
\label{sec:AE}

\begin{com}

All reviewers agreed that your work has potential but raised significant concerns, in terms of definition, presentation, and evaluation data. Please see detailed comments below. 

\end{com}

We would like to thank all our reviewers for their extensive feedback. As part of major revision, these are some of the changes which can be observed in our paper. We have formatted our structure to make it look like an empirical study on the recommendation of Reviewer 2. We have added another figure for our RQ1  to address the concerns of Reviewer 1. Please look at our replies to them below. As for Reviewer 3, their comment were insightful and lead to significant changes
throughout the paper.

\subsection*{Reviewer 1}
\label{sec:Reviewer1}
\renewcommand*{\theenumi}{1.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}

\be 
\item \begin{com}
$>>$ Summary $<<$

This paper aims to reduce the complexity of hyperparameter optimization for software analytics by focusing on 2 tasks (defect prediction and bug report text mining).

This paper proposed an approach by discretizing the spaces of exploration into $1/(\mathcal{E}^2)$ groups to avoid exploring any redundant parameter settings. The results show that \IT* outperforms many baselines algorithms for 2 SE tasks.

$>>$ Evaluation $<<$

I enjoy reading the manuscript. The paper addresses an important topic in software engineering where the goal is to make software analytics algorithms faster. Please kindly consider addressing my detailed feedback. Most of them are clarification questions, not a critical concern. I hope that my feedback will greatly improve the manuscript prior to recommending acceptance. 
\end{com}

Thank you for your support to our work. We have provided a detailed feedback to your concerns below.

\item \begin{com}
$>>$ Detailed Feedback $<<$

- I find the ``complexity / simpler'' terms that are used in the paper are a bit slightly misleading. When referring to the complexity, I was thinking about the complexity of defect models (which can be measured in terms of \#variables used in the model). However, this paper seems to focus on the speed of the model building. 

- Later on, the authors stated that ``simpler means less CPU is required to build better software quality prediction models". Should the keyword be changed or not in order to ensure that the paper is properly scoped? E.g., changing ``simpler" to ``faster"? Less claim and more straightforward.
\end{com}


We agree to your suggestion, by changing "simpler" to more precise
terms (e.g. ``faster''), we have now focused more on how \IT* makes software analytics easier.

\item \begin{com}
- In Introduction, ``Software analytics is becoming increasingly complicated.''. Please be more explicit and specific in what aspect that it is more complicated (e.g., modelling design, parameter settings, data cleaning, infra, mining, execution time)?. And what aspect that this paper is focusing on.
\end{com}


We agree that that first sentence lacked definition. We have deleted it.
Now we motivate out work as per the Fisher et al quote (i.e. we want to make things faster). 
With this in mind, faster iteration is important. Here we focused on exploring billions of parameter settings to find optimal settings faster.


\item \begin{com}
- ``FFtrees [42] outperforms the supposed state-of-the-art SE tuning algorithms''. I read this sentence like FFtrees are an optimization algorithm (e.g., DE, random search), but I do believe it is not. 
\end{com}

Good point. We have significantly modified that sentence
(see the new introduction).



\item \begin{com}
- In Introduction (RQ2) (and throughout the paper), when saying outperforms, could you please elaborate more about the magnitude of the (absolute, not relative) improvement? 

- ``\IT* generates better quality predictors than ...''. Again, could you please elaborate more how they are better, what aspects that DODGE is better (accuracy, speed, F-measure), and how much.
\end{com}

Excellent point. We have fixed- See updated RQ2 text in the introduction.


% We have updated the text in the paper (see the new RQ2 text).
% . We showed that  We show that {\IT*}   out-performs for the defect prediction study as below:
% \bi
% \item An ICSE'15 article that explored many different learners for
% defect prediction~\cite{ghotra2015revisiting} by about 50\% and 40\% on an average for {\em d2h} and {\em Popt(20)} respectively;
% \item
% An IST'16 journal article that demonstrated
% the value of  tuning
% for defect predictors~\cite{fu2016tuning} by about 30\% and 10\% on an average for {\em d2h} and {\em Popt(20)} respectively while exploring larger parameter search space with faster termination;
% \item
% An ICSE'18 article that advocated     tuning  data pre-preprocessors~\cite{agrawal2018better} by about 10\% and 5\% on an average for {\em d2h} and {\em Popt(20)} respectively while exploring larger parameter search space with faster termination.
% \item
% The FSE'18 article that reported the FFtree results~\cite{chen2018applications} by about 10\% and 5\% on an average for {\em d2h} and {\em Popt(20)} respectively while exploring larger parameter search space with faster termination.
% \ei

% For   text mining, we show 
% {\IT*} performs better than:
% \bi

% \item
% An IST'18 journal article that had showed the value 
% of tuning for SE text mining applications~\cite{agrawal2018wrong}  by about 20\% on an average for {\em d2h} while exploring larger parameter search space with faster termination.
% \item
% An earlier ICSE'13 article that applied genetic algorithms to
% learn the settings for a text miner~\cite{Panichella:2013} by about 20\% on an average for {\em d2h} while exploring larger parameter search space with faster termination..
% \ei

\item \begin{com}
- When endorsing DODGE over FFTrees, I'm concerned that the authors miss the key aspects of FFTrees (interpretable and comprehensible). Should these 2 aspects be considered when strongly recommending DODGE over FFTrees? 
\end{com}

You raise an important point and we added a note to that effect,
third last para of introduction. 

That said,  more fundamentally, the other reason to explore {\IT*} is that it tests the theory that much better hyperparameter optimizers can be built by assuming the  output space divides into just
a few regions of size 
  $\mathcal{E}$. {\IT*} is one way to exploit this effect.
  We believe that  further research could be done to supercharge {\IT*} by incorporating other information inside, for e.g., preferences on few learners over others; better visualizations and/or explanations of analytics.

% And to expand a little on this point: we agree that FFTrees are shown to be more interpretable and comprehensible, and in the current framework of \IT*, it doesn't incorporate the goal of interpretability. We wanted to stress on 2 things which was found after the introduction of \IT*, they are: 1) Software Analytics is different that studies problems with large $\mathcal{E}$ and it can be utilized to make hyperparameter tuning faster and better; 2) \IT* explores billions of choices of preprocessors and learners at the same time (from Table~\ref{tbl:options}) which no other hyperparameter tuning tool explores. Also \IT* does it better and faster than other hyperparameter tuning tools.

% But we would like to say that there are information like interpretability or runtimes that can be included in the \IT* to supercharge the search. For e.g., Decision Tree (DT) and Random forest (RF) can generate trees which are interpretable and actionable so we can assign higher initial weights to DT or RF in \IT*. That way we can get interepretable models too. Though this is a future exploration which we want to carry out.

\item \begin{com}
- When the authors argued that DODGE is simpler (which is faster) than FFTrees, I'm curious if DODGE gives a higher accuracy in terms of predictions or not. Simpler but lower accuracy might not be a good predictor. More clarification with a stronger statement would be appreciated.
\end{com}
 
 
We are not clear on this point.
Most    SE analytics papers do not report accuracy since it  can be very uninformative
on SE datasets. A  predictor for a data set where
20\% of its rows contain the target class can be   80\% accurate while missing all the target. Our preferred measures
for such data sets are things like d2h, or something that captures the business
case for the analytics such as Popt(20).

And measured on this values \IT* gets higher performance with faster terminations. Please look at our reply for 1.5.  

\item \begin{com}- In Introduction, ``our approach needs to be tested using more SE tasks'' -$>$ and more SE datasets as well. I have a big concern about the current defect datasets (e.g., Log4J 1.2 has a 92\% defective ratio, Xalan 2.7 has a 99\% defective ratio). Would a simple Zero Rule algorithm outperforms DODGE or FFTree in the context of transfer learning or cross-project defect prediction?

%\url{https://machinelearningmastery.com/implement-baseline-machine-learning-algorithms-scratch-python/}
\end{com}

 
ZeroR is ``too blunt an axe'' for this work. FYI, We originally included
it in the Table~\ref{tbl:options} learners list but it performed so poorly that we took it out.

You can see why it performed so badly,   looking at the training/test columns of Table~\ref{tbl:versions}:
\bi
\item
Observe
how, in that table, two of the data sets have defect densities higher than 50\%.
\item
For those data sets (Lucene and Velocity)
hyperparameter optimization (optimizing for d2h) would select for ZeroR.
\item
Such a selection would
lead to poor results
half the time. In their testing dataset versions, Lucene and Velocity have 60\% and 34\%
defects which means that, for that data,
ZeroR would have incorrectly classified 40\% of Lucene and 66\% of Velocity.
\ei
 


\vspace{2mm}

Also, note that ZeroR  does not address the core business case of defect prediction.
In safety or mission-critical software, it is ok to demand the engineers to
inspect all the code. But most software is not mission/safety critical
so engineers seek heuristics to reduce their inspection effort.
As stated by 
Ostrand and Weyeuker in 2004~\cite{ostrand2004bugs},
Arisholm and Briand in 2006~\cite{Arisholm:2006}, 
Menzies in 2007~\cite{menzies2007data},
the 
business goal of defect prediction is to avoid inspecting everything. So
we use defect predictors to 
find the smallest part of the code containing
most errors. 
In fact, when researchers report the industrial impact of defect
prediction, that impact is usually expressed in financial terms
of reduced inspection effort.
Tosun et al.  (2011) reported that defect prediction reduced  inspection efforts by 72 percent~\cite{mirirli11} (without damaging defect detection rate).
Kim et al. (2015)  also found that defect predictions
reduces the  resources required for tests, again without damaging defect 
prediction~\cite{Kim:2015}.

\vspace{2mm}

Well (you may ask), if reducing inspection effort is so important, why isn't that including in the evaluation metrics? Well (we reply), it is. Popt(20) reports
what happens when you let the defect predictor guide you to a small portion
(20\%) of the code. 
 


\item \begin{com}
- Section 2.2, ``Our defect predictors use static code measurements from Table 2 (now table 5)  and Table 3 (now table 6).'' Table 3 is not defect predictors. Please revise to ``Statistics of the studied data sets.''
\end{com}

Fixed! Thanks for point that out.

\item \begin{com}
- "For example, we use poi1.5,poi2.0,poi2.5 data for training predictors". I'm concerned if this will introduce any biases to the learning algorithms due to duplicate signals or not. For example, File A.java appears in poi1.5, poi2.0, and poi2.5 but they have 3 rows in the training data where some of them could be either defective or clean. I would like to see your view/rationale/discussion on this. Would this be a threat to construct validity?
\end{com}

You make an important point since it speaks to the nature of machine
learning (and while early progress was so slow and why
later work was so successful).  A learner watches the environment
and receives signals from artifacts in the field. Early work in machine
learning performed very poorly since it obsessed too much on
single examples. Later, new better work know how to handle noise
and how to average out its conclusions
over multiple samples. To return to your example, if FileA was defective, not defective, defective in poi1.5 and poi2.0 and poi2.5 (respectively)
then a leaner would know not to use the attributes ranges seen in those entries to make its conclusions. 

% That is right, it will be a threat to construct validity. We know different algorithms could have different bias due to various threats to validity. For any empirical study it is needed to verify and validate our methods using multiple datasets, for multiple case studies. We verified our framework \IT* against 2 case studies on about 16 datasets, reducing any threats to this study further. Though we added a section on construct validity in the paper in Section~\ref{sect:threats}.

\item \begin{com}
- Table 3 (now table 6), the 3rd column, please be specific whether they are a defective ratio of which software version? There are 3 software versions but the authors report only one ratio.
\end{com}

Thank you for asking that question. We have fixed the caption of that
figure to clarify that point.

And to answer your question: 
the defective ratio represents the combination of total defective ratio after combining all the software versions used for training. That is why we reported only one ratio.

\item \begin{com}
- "This tells us that software analytics will forever be an imprecise science (and one of the lessons of this paper is that imprecision can be used to simplify complex tasks like hyperparameter optimization)." Is this argument necessary? I have a big concern with the "Imprecise Science" term. I do not see how the higher defective ratios in later software releases lead to the conclusion of "imprecise science". They are just the dynamism in software development projects without any relationship to imprecise science.
\end{com}

Thanks for picking up on that. That was a silly sentence which we have deleted.


%%%XXX

\item \begin{com}
- "Table 5 FFTree reference four attributes cbo, rfc, dam, amc (defined in Table 2)." Do the four attributes are selected by FFTree or subjectively selected by the authors? Is the number of attributes a part of parameter setting for FFTree? What is the impact when varying this parameter?
\end{com}

They are selected automatically by FFtrees. 

These 4 attributes were selected by FFTree. FFTree has a parameter which represents the depth of the tree, whatever the depth would be that many attributes would be selected. In our case it is 4. We did explore the depth equal to 5, and 6 but we did not find any improvement against the depth of 4. So, we consistently used this parameter to compare our other frameworks. Also, Chen et al.~\cite{chen2018applications} also found that depth of 4 works as best as other settings.

\item \begin{com}
- In Section 2.3.1, the d2h measure is proposed by the authors. Could you please provide the rationale behind the d2h measure? What does it directly measure? Why combining these 2 measures instead of the others? Please include AUROC or MCC as well, as they are less susceptible to skew/imbalanced data.
\end{com}

(Aside for your information, $d2h$ is not proposed by this paper-- it has been a standard measure since first  introduced in 2007.)

Your question raises an interesting point.
We use recall and false alarm (summarized via $d2h$) exactly
{\em because of} the skew/imbalance problem you mention.
We use recall and false alarm
since they have few problems with
skewed/imbalanced data\footnote{In 2007 we published a mathematical and empirical
study on the skew/imbalance problem. We found that accuracy and precision have
certain undesirable properties~\cite{Menzies:2007prec} (very steep partial differentials across goal space) that leads to conclusion
instability in certain
cases that are common in SE
(the skew/imbalanced data that you mentioned).}.
And the same has not been shown (yet) for other measures.


As to what $d2h$  means, an ideal predictor would have perfect recall (it would find all the target)
and have no false alarms (it would make no mistakes).
In terms of a recall/false alarm trade-off, that would be the ``heaven''
point of recall=1 and false alarm=0. That is,   distance to heaven
measures how close you are coming to perfection.


As to  why not MCC, well, that comes for a private comment Martin Shepperd shared with us-- MCC has a strange double-hump non-Gaussian property that is worthy of a paper all itself (something like~\cite{Menzies:2007prec}). 




\item \begin{com}
- "We call these learners "standard"" -$>$ Should the authors call 'baseline learners' instead? 
\end{com}

Recently in TOSEM'18, Federica Sarro proposed a nine-point
definition of baselines (see table1 of http://bit.ly/2IXWxQl).
That is "baseline" has become a reserved term which we might not be to apply in the ways you suggest. 

In fact, we have taken care to remove the word ``baseline'' entirely from this paper.

\item \begin{com}
- Fig 4, "keeping samples constant at N = 30.". What does it mean? I do not follow. 

- Fig 4, why "small effect = 4.4? What does it mean?

- Fig 4, what is the X-axis? 
\end{com}

Keeping N=30 means we never evaluated options within {\IT*} more than 30 times. Fig 4 is now Fig~\ref{fig:varE}  where (in the caption) now we say "evaluations".

(Aside: and to answer the question ``why did we pick N=30'', we refer you to \fig{varN} were we found no value in increasing $N$ to much larger values.)

%When we say "keeping samples constant at $N=30$." Please see Figure~\ref{fig:motivate_quickly} and RQ1 updated text where we explained it. 

%(and note in This says that we report the performance of \IT* for different $\mathcal{E}$ values after terminating at $N=30$ evaluations.

 
Fig 4 is now Fig~\ref{fig:varE} where X-axis represents $d2h$ and $P_{opt}$ values. 

When we say small effect, we used stats test of Cohen's delta~\cite{cohen1988statistical} defined in Equation~\ref{eq:cohen} defined in section 2.3.2.
The cohen's delta for different $\mathcal{E}$ values understudy give us a value of 4.4 and statistically it means the difference is of small effect or insignificant.
%%% Add the figure to explain further.


\item \begin{com}
- Section 4.1, please clearly describe what settings that are explored for {N, e}. I'm missing this part. The authors only explore different e, while keeping N constant, or explore the variations of both parameters. 

- It would be nice if the authors combine Figure 4 and 5 as a trade-off analysis plot where the plots truly demonstrate which parameters are the best. At the moment, it seems like they are individually assessed.
\end{com}

We have modified our text in \tion{rq1} explaining these 2 figures more in detail. Please see the explanation of both figures below as well:
\bi
\item \fig{varE} varies  $\mathcal{E}$   but keeps $N$ constant. Please note, when we say $N$ constant, we wanted to see how much improvement do we miss on when we try to find the right $\mathcal{E}$ value. Let's say we cut the Figure~\ref{fig:motivate_quickly} at $N=30$ line on x-axis, we report the values of  $\mathcal{E}$ for 0.05, 0.1 and 0.2.
\item \fig{varN} varies $N$ but keeps $\mathcal{E}$ constant. Please note, when we say $\mathcal{E}$ constant, we wanted to see how much improvement do we miss on when we try to find the right $N$ value. Let's say we look at $\mathcal{E}=0.2$ line, we report the values of  $N$ for 30, 100 and 1000.
\ei

These 2 parameters are actually not assessed individually. In another outlook, we provided another Figure~\ref{fig:motivate_quickly} in the text showing how the values of Figures~\ref{fig:varE} and~\ref{fig:varN} are derived from Figure~\ref{fig:motivate_quickly} while assessing them at the same time. If you look at figure~\ref{fig:motivate_quickly}, we observed that there is not significant loss in performance if we move $\mathcal{E}$ to different values or $N$ provided in figures~\ref{fig:varE} and~\ref{fig:varN}. At the end of RQ1, we picked $\mathcal{E}=0.2$ as we are looking for larger redundant region in data at the same time faster evaluations of $N=30$.

\item \begin{com}
- Is \IT* specific to FFtrees or any classification techniques? I had a perception that DODGE is for any learning algorithms, but in Section 4.1 I read like DODGE is only for FFTree (e.g., "while taking N = 30 samples of the options tree."). 

This question is really important if DODGE is at the foundational role of software analytics or DODGE is limited to one specific single classification algorithm (i.e., FFTree). 


Now, I will interpret DODGE as FFtree+Optimizer, which is just one classification technique. If so, please clearly specify at the beginning as I'm not too clear about what DODGE is when reading the introduction section.
\end{com}

Your initial perception is right. \IT* is for any learning algorithm. It finds the optimal learning algorithm with its parameter settings all simultaneously from bunch of options as shown in Table~\ref{tbl:options}. When we said, "while taking N = 30 samples of the options tree.", we wanted to say options from Table~\ref{tbl:options}. We have modified the text in the paper.

\item \begin{com}
- There are some threats to the internal validity that can be discussed .
\end{com}

At your suggestion we have extended the threats to validity section  Section~\ref{sect:threats}. 

\item \begin{com}
- "machine learning algorithm developed in the AI community might not apply to SE." It would be nice to add an example as this argument has been raised in prior work (Fig 1) where they find that RF that is the top-performing in the ML area, but sometimes they are not for some SE datasets. 
\end{com}

Thank you for your suggestion, we have added the example in the paper (see last page
of conclusion).

\item \begin{com}
$>>$ Typo $<<$

(numerous typos listed). 
\end{com}

We have fixed the above typos and any other typos which we could have identified.

\ee


\subsection*{Reviewer 2}
\label{sec:Reviewer2}
\renewcommand*{\theenumi}{2.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}

Thank you for your close reading of the text, and your excellent suggestions. As you can see, based on your remarks,
we have made major changes to the overall
structure of the paper as well as numerous other (smaller scale) changes around the paper.



\be 
\item \begin{com}
Finding a good tuning for software analytics can be a big challenge. Analytics tools often make use of machine learning with plenty of hyperparameters to tune, but often default parameter settings are used. Previous research shows that finding a good tuning can drastically improve the results from analytics tools. The lack of tuning in parts of previous research raises the question if conclusions from comparative studies from the past would still be valid if proper tuning would have been done.

In this paper, the authors present DODGE, a pragmatic tool for hyperparameter optimization. The main feature of DODGE is that it ignores redundant settings, thus it operates much faster than an exhaustive search. Still, results from tuning of defect prediction models and text mining show that DODGE can deliver better tunings than algorithms presented in previous work.

The manuscript addresses an important topic and contributes novel insights that could support the software engineering community. If the authors document how to use DODGE (in a comprehensible way), I believe this work could have an academic impact. Reading the manuscript convinces me that the authors have substantial experience from hyperparameter optimization of various machine learning models. Also, the application of DODGE on two different applications, i.e., defect prediction and text mining, supports the argumentation in the paper very well.
While I enjoyed reading the manuscript, I think it needs a major revision before being published in a flagship software engineering journal. I have two major considerations that should be addressed.
\end{com}

Thank you for your support, we have addressed your concerns below.

\item \begin{com}
First, I don’t think the writing style is suitable for a top SE journal. While partly a matter of taste, I think a revised version could help future readers. The manuscript alternates between a casual language suitable for a blog post (e.g., parts of the introduction) with content that is hard to digest (e.g., Table 1). I recommend the authors to revise the manuscript with the readership in mind. This could result in a more academic writing style in some parts of the paper and improved explanations to help the reader digest the technical parts – perhaps also adding some figures with concrete examples to illustrate DODGE and FFTree. Since the paper has an important message to communicate, I recommend the authors to consult a professional copy editor to improve readability and fitness for its purpose.

Moreover, the manuscript does not follow the conventional IMRAD structure of a research article. While this certainly is not a requirement, I think the authors should think about whether the current structure really is a better option. To me, the structure of the manuscript increased the cognitive load instead of supporting my reading experience. My guess is that the authors want to frame the paper as an experience report rather than an empirical study, but I don’t think this is the right choice for a TSE paper.
\end{com}

%%% XXX Suggestions here?
Thank you giving us the insight on the structure of the paper. Based on your recommendations, we have completely modified the structure of this paper.

Now we follow, as you suggest the structure of
 Introduction, Related work (section2), Motivation (section3), method (section4) and experimental results (section5) .
 
We have also added a Figure~\ref{fig:tabu_pseudo} explaining \IT* and there is an example of FFtree in Table~\ref{tbl:three}. %Since, fftree is coming from Chen et al.~\cite{chen2018applications} implementation, we only provided a small snippet of an example and a small desciption of how fftree works. Please let us know if you have further comments.

\item \begin{com}
Second, I miss a proper related work section in the paper. The challenge of hyperparameter tuning is not unique to software analytics. I support the authors’ decision to focus only on SE in this manuscript, but I think the background and/or related work section should introduce the reader to work on tuning also beyond SE. It is good to see that the authors compare DODGE to other hyperparameter optimization results from prominent SE venues, but I think a TSE paper should also synthesize the general discussion on the hunt for feasible parameter settings – this would also turn the paper into a stronger contribution within SE, i.e., it would balance the heavy component of machine learning details. 
\end{com}

%%% XXX Suggestions here?
Excellent suggestion! Please see \tion{related}.

\item \begin{com}
I understand that the authors decided not to compare DODGE to optimizers from search-based SE, but I think the authors should still discuss parameter tuning in the light of previous work. A quick search for related work using a few keywords gave me: 
i) Arcuri, A., \& Fraser, G. (2013). Parameter tuning or default values? An empirical investigation in search-based software engineering. Empirical Software Engineering, 18(3), 594-623, 
ii) Altinger, H., Herbold, S., Schneemann, F., Grabowski, J., \& Wotawa, F. (2017, February). 
Performance tuning for automotive software fault prediction. In 2017 IEEE 24th International Conference on Software Analysis, Evolution and Reengineering (SANER) (pp. 526-530), 
iii) Borg, M. (2016). 
TuneR: a framework for tuning software engineering tools with hands‐on instructions in R. Journal of software: Evolution and Process, 28(6), 427-459, and 
iv) Aleti, A., Moser, I., \& Grunske, L. (2017). Analysing the fitness landscape of search-based software testing problems. Automated Software Engineering, 24(3), 603-621.
\end{com}

Thank you for finding those references. We have extended the Related Work section as you suggested
(discussing the relationship of {\IT*} work to others). 

If you don't mind, we'd rather not include papers from SANER and SEP
but the ASE conference and journal papers you mention are now added to the literature review. Also, we traced forward in time
and found some interesting subsequent work that offered extra insight into Arcuri et al.

As to your more general point, that there is much more that could be said about this topic, we agree. 
Please see our latest literature
review  on this topic; e.g. https://arxiv.org/pdf/1812.01550.pdf (currently under review, second round, at EMSE).
Our new related work section (\tion{related}) references that paper (and gives a link for free download).



%%% XXX Suggestions here?

\item \begin{com}
Detailed comments:

Abstract: The abstract needs to be revised. It contains a mix of very short and very long sentences, unconventional use of parentheses and quotation marks, and the first sentences led me to expect a different contribution in the paper. The “AI software” mentioned first is not about software products enabled by AI (e.g., a classifier trained for object detection in a self-driving car), but rather software analytics tools used by software engineers to support development of high-quality software products. At least I was confused by how the paper started. 
\end{com}

Thank you for your suggestion, we have updated the abstract. 

\item \begin{com}

Page 2:19 – The paper never defines what is meant by software analytics. Do the authors include anything related to analyzing software product and process data? 
\end{com}

Please see the first line of the new introduction.  And yes, analytics includes anything related to analyzing software product and process data.
 

\item \begin{com}
Table 1: I fear that the table would shock the reader early on with very many terms without any explanation. I suggest keeping only some of them, explaining them carefully, and then moving the rest to the appendix.
Figure 1: This caption might be too long. Perhaps move parts to the running text?
\end{com}

We've done as you suggested and moved some of the caption text into page1 of the introduction.
But
if you don't  mind, we'd rather keep the rest  where it is. the whole point of that in the paper is, as you say, to shock
the reader into realizing how large and complex is the internal choices of all these machine learners. 
 
\item \begin{com}

Page 4:46 – “assessment effectiveness increases exponentially with assessment effort” Is there a typo here? I guess the effectiveness of QA rather saturates, at least in terms of identified bugs. I might misunderstand the statement.
\end{com}

Thanks for catching that. We've fixed that now to ``Software quality assurance budgets are finite but increasing assessment effectiveness by some
 linear amount can take   exponentially more effort.''.
 
\item \begin{com}
Page 5:5 – “predict 87 percent of code defects”. What is the granularity here? File? Or method? Important to clarify.
Table 3: Same as above. What does “\% of defects” mean?
\end{com}

Clarified now in text: When Misirli et al.~\cite{misirli2011ai} built a  defect prediction model  for a telecommunications company, those  models
could  predict 87\% of files with  defects.
 

\item \begin{com}
Page 5:37 – The time dimension is interesting and cross-validation might lead to overly optimistic results. Two papers discussing this “Online Defect Prediction for Imbalanced Data” Tan et al., ICSE2015 and “Automated Bug Assignment: Ensemble-based Machine Learning in Large Scale Industrial Contexts” Jonsson et al., EMSE 21(4), 2016.
\end{com}

 If we understand you correctly,  you are saying that we did cross validation on defect prediction datasets.
 But this {\em not} what we did. 
 For defect prediction,
 we had access to multiple versions of software so we used past releases as training and the most recent one as testing data.

% That might be true but our conclusions are not about the predictors, per se, but about the relative merits
% of different optimizers trying to solve some task using some learners. As long as we keep the task constant (and that 
% could be done with cross-val, or with temporal) then we can compare our different optimization/hyperparameter optimization
% strateggies.

\item \begin{com}
Table 2: The code metrics are not explained. Perhaps add explanations in an appendix?
\end{com}

We will ask the AE about that (but last we checked TSE does not allow an appendix). Meanwhile we have updated the caption of Table~\ref{tbl:ck} to refer \cite{agrawal2018better} for the definitions.

\item \begin{com}
Table 4: Very many acronyms introduced here. Perhaps better to explain the four groups in running text and add a reference to Ghotra et al. for details? Presenting such complex details without explaining them might not be the best choice from a readability perspective.
\end{com}

We agree and based on your recommendations we have removed the table and provided a reference to Ghotra et al. in the text.

\item \begin{com}
Page 6: I like the metrics!
Sec 5: The critical discussion in the manuscript is brief and solely addresses external validity. There might be additional aspect to discuss in this section. If important control parameters are not explored, is that really an external validity threat? Wouldn’t that rather be a confounding factor? Regarding construct validity, I’m thinking about whether binary severity prediction is a meaningful construct. On the other hand, that is not the main point in this manuscript. 
\end{com}

As noted in the beginning of our replies to you, yes, that is not the main point of this paper.
Your remarks have also highlighted for us a structural flaw in the previous version.
To make the main point clearer,
we have added the following into the text of paper.

IN THREATS TO VALIDITY, we now say: This paper is not about how to generate good predictors, per se. Instead, it is more  about  an instrument, {\IT*}, that probes the nature of the 
space options associated with  AI tools applied to SE. We show that when prior work has tried to generate good predictors, their algorithms have been much slower
than necessary since those algorithm have wasted much time exploring a vast amount of redundant options.
To show that, we repeat numerous prior studies, this time adding in {\IT*} framework.  
Since we are repeating prior work, 
our work shares the same threats to validity as that prior work (such is the nature of repeated studies).

% IN THE CONCLUSION,  we now say: 
% This paper is more than jsut a ``replicate-with-some-tweaks'' study.
% Where this work  significantly {\em extends} prior work is that we  show that  similar.  (or better) results can be obtained (much faster) using another kind of tools that is aware (and avoids)   redundancies in the search space for good hyperparameters. 
% Also, where this work could {\em inspire} much future work  is as follows.
% Once  researchers move from CPU-intensive methods to  CPU-light methods  (e.g. that avoid redundant options)
% then a much broader range of choices could be explored and much better predictors could be created by future work.



\item \begin{com}
Nitpicks:

(numerous typos listed)
\end{com}

We have fixed the above typos and any other typos which we could have identified.
\ee



\subsection*{Reviewer 3}
\label{sec:Reviewer3}
\renewcommand*{\theenumi}{3.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}

\be 
\item \begin{com}

This paper introduced a hyperparameter optimization tool named DODGE to ignore redundant tunings and can run orders of magnitude faster. The performance of DODGE can find better tunings than state-of-the-art techniques. They evaluate their tool on two software tasks, namely, software defect prediction and software text mining.  The authors give detailed introduction of its baselines and their results. I consider the problem address in this paper to be relevant, and the approach presented innovative. I would like to see the contribution of your work built on by going into more depth in each component of your approach. Currently, the presentation of your approach and its baselines are mixed.
\end{com}

Thank you for your supporting words. We have addressed your concerns below.

\item \begin{com}
Specific suggestions for each aspect of the paper are given below:

I have some concerns about the evaluation that cannot be ignored. 
The first concern is the details of DODGE. The author describes the baseline FFTree in detail. However, it is hard for the readers to assess the percentage of original contribution from your side, from the percentage of use of existent work.  
\end{com}


You are correct-- the prior draft contained no section ``relation to prior work''. That was out mistake,
which we have fixed in this draft. 
Please see the new \tion{prior}.

% We  mentioned our contributions at the end of the introudction section in terms of multiple RQs and final list of what have we achieved. We showed that we contributed \IT* as part of the new framework and compared results against many baseline methods of \cite{agrawal2018wrong,agrawal2018better,chen2018applications,Panichella:2013,fu2016tuning,ghotra2015revisiting}. 

% As for better
% understanding the FFtree algoirth
% We described FFtree in detail as the results presented by Chen et al.~\cite{chen2018applications} motivated this article, giving us our framework, \IT*. We have also expanded the details in the section~\ref{sect:dodge} with another figure~\ref{fig:tabu_pseudo} introducing its pseudocode.


\item \begin{com}
The second concern is about the organization and presentation of the experiments. It is rather confusing with details about the experiment spread between Section 2 to Section 4. For examples, the RQs are proposed in Section 1.  In particular, the RQs should be presented first and then all the details of the design of the experiment adopted to answer these RQs, including the used baselines, the dataset, the way the dataset has been used to build the model, the metrics to answer the RQs, and so on.
\end{com}

You raise an important point.
If papers follow a standard structure then
that reduces the effort 
required by humans to skim and understand a paper.

Accordingly,
based on your recommendations and reviewer 2's suggestions, we have changed our structure of the paper to provide better readability.
To that end, we have adopted a more standard
structure for this paper:

\bi
\item
All  our RQs are now introduced in 
the introduction.
\item
The  paper now follows the standard
structure of  
 Introduction, Related work (section2), Motivation (section3), methods (section4) and experimental results (section5).
\ei 

\item \begin{com}
The author should give the definition of $\mathcal{E}$ first, it is important for the readers to understand the approach better. In addition, it is unclear how does the \IT* work. The authors should introduce their approach in detail.
\end{com}


We have now provided a definition on $\mathcal{E}$ in the introduction section. We have also expanded the details in the section~\ref{sect:dodge} and with another Figure~\ref{fig:tabu_pseudo} introducing its pseudocode in detail.

\item \begin{com}
Page 1. What does the output space mean? 
\end{com}

Our mistake-- we did not define that term
when we first used it.
That has now been fixed (see page1).
FYI:  a learner assessed by $p$ performance scores has a $p$ dimensional output space.

\item \begin{com}
Page 2. There is a figure without label on right column. This figure also lacks more details. At least,   how can you get the 25 cells from the figure.
\end{com}

You are correct to point this out. We have added a label to that figure.
The 25 cells in the Page1 figure comes from the 
calculation
$1/\mathcal{E}^p=1/{0.2}^2=25$, where $p$ is the number of performance scores.  

\item \begin{com}
Page 2 line 9. It seems that unclear for what the authors want to give us examples in the abstract. 
\end{com}

Your are right. Example now removed. 

\item \begin{com}
Page 3. In Table 1, the authors listed some traditional learners. But neural network-based models are not mentioned, whose performance also depended on the hyperparameters.
\end{com}

You are correct. Table~1 is not complete-- something we did not stress in the original version (but now we do, please see the first \textcolor{red}{red text} on page1.

Note that this paper does not need to explore
{\em all options}-- it just needs to explore
the common ones seen in the analytics literature.

As to the specifics of neural nets, whenever
we've explored them for  SE analytics, we've found
simpler, faster, and better alternatives \cite{majumder18,fu2017easy}.
Others researchers
have had similar experiences~\cite{hellendoorn2017deep}.

\item \begin{com}
Page 3. In Figure 1, the authors said that “Y-axis shows the frequency at which a learner was selected to be “top-ranked” (by a statistical analysis)”. What does “top-ranked” mean? Does it mean that this learner performs best? 
\end{com}

We have removed that figure.

\item \begin{com}
Page 4. The authors didn’t explain why the FFtrees used fewer evaluation.
\end{com}

Excellent point! We never closed
that loop. Please see the new \textcolor{red}{red text}
  at start of conclusion. 

\item \begin{com}
Page4. It is hard to understand how to get the results of Figure 2. It is better to add more details of this figure.
\end{com}

Sorry about that . The figure2 text has been clarified and  improved.
 

\item \begin{com}
Page5 line 34. What does the phrase “those methods” mean? I can’t find any description of those methods. 
\end{com}

We cannot find that text in this version. Perhaps
it was deleted during an edit about some
other point.
 
\item \begin{com}
Page 5 line 47. How to get the median defect percentage in training data is 29\% and in the test data, it is49\%? It seems not 49\% in test set.
\end{com}

Our mistake, the median is 52, not 49, calculated as follows.
The test set numbers are

2,11,19,34,34,69,64,74,92,99

The median is half way between 34 and 69 i.e. 52.
 

\item \begin{com}
Section 2.3.1. The authors give many reasons which are popular in prior works but not suitable in these tasks, such as precision or accuracy. They should give the advantages of the proposed metrics d2h and Popt. It is important to expound if it is reasonable of the metrics. It would be better to explain them with examples. 
\end{com}

Thank you for that suggestion. Please see new text, start of \tion{easures}. Also, please see our reply to reviewer1.14.
Note that we do not elaborate on our reasons for not using precision-- that
would require a more lengthy explanation,
which we have  published previously (see~\cite{Menzies:2007prec}).

%%%XXX

\item \begin{com}
Page 6 line 17. The author thought the large variation in the out space caused the mentioned conditions. Is there any evidence can support this hypothesis? What will happen if there are enough data and the margin between training set and testing set is little?
\end{com}

We have been seeing many such examples from the past where only few key evaluations can provide better measures. For e.g.,
\bi
\item Feature selection results of where two to three attributes was enough to predict software defects
or development effort~\cite{menzies2007data,chen2005finding,menzies2003data}.
\item Incremental learning results of~\cite{menzies2008implications,menzies2010defect} where 
a few dozen examples of defective and non-defective modules
performed as well as anything else.
\item Maths model at the end of~\cite{nam2017heterogeneous} that showed, in the expected
case, that very few examples are required to learn
SE defect models.
\ei

But till now there hasn't been any explanation or a way to utilize this large variability in the data. \IT* is a framework which also provided the explanation and existence of this large variation without the need of any other past evidences.

We do believe if there are enough data and the margin between training set and testing set is little, then this framework might or might not work. We are still exploring this as part of future work.

\item \begin{com}
Section 2.4. “We first used them as an explanation tool, but realized that they had broader implications.”  Would you please give some implications for better understanding?
\end{com}

We deleted that sentence (irrelevant to this article).

\item \begin{com}
Section4.1 page 8. The author didn’t give the reason why N=30 and ε=0.2. Also, Why N is evaluated among 30, 100, 1000 and ε is evaluated among 0.05, 0.1, 0.2.  In figure 4, it seems better when ε = 0.05 than ε =0.2.  In figure 5, the results of N=1000 outperform N=30. The author may provide more details for answering RQ1.
\end{com}

You are right, that was not explained enough in the text. We now updated more details in the RQ1.
When tested with an effect size test we could not show
that 
the delta between N=30 and N=1000 was statistically supportable. 
Note that the text in \tion{rq1} now says {\em As shown in these figures, these changes to $\{N,\mathcal{E}\}$ alter the performance of \IT* by less than a ``small effect''.}



\item \begin{com}
Section 4.2. This paper just describes the results of DODGE(0.2) and baselines. I am more curious why is DODGE better/worse than the baselines.  In addition, why is the DODGE worse than baselines when it was measured be D2h while better than baselines when it was measured by Popt. 
\end{com}

As to your first point, please see the new text at start of conclusion.

As to your second point, 
we added more text to explain that. Top of \fig{smote}
we point that that {\em smaller} values of $d2h$ are better
while {\em larger} values of {\em Popt(20)} are better.
That is, on both measures, usually  {\IT*} performs better. 
Note that we also stress that, earlier in the paper, when we define these measures
(see text at end of \tion{easures}).

% Fig~\ref{fig:smote} provides result for defect prediction where we showed \IT{.2} performs better than other baselines. We want to clarify, that \IT* performs better than baselines for both the measures, $d2h$ and $P_{opt}$. We have provided more details in the text of the paper. When we say \IT* performs better we mean statistically either they are significant better or similar than any other baselines. For Fig~\ref{fig:smote}, \IT* wins in 16 out of 20 datasets when combined for both the metrics. \IT* wins by on an average of 10\% and 5\% for $d2h$ and $P_{opt}$ metrics respectively for both SMOTUNED and FFtrees.


\item \begin{com}
Section 4.3. The authors introduce the algorithms for text mining in detail, i.e., SVM and LDA. What does DODGE do in the text mining task? It seems unclear here. The author should give explanation further.
\end{com}

Good point. Please see the first text in \textcolor{red}{red} at start of \tion{text}.
\IT* is an optimization tool which can tune the parameters of transformation (LDA) and learner (SVM) at the same time. \IT* explores the billions of options created from Table~\ref{tbl:options} when combined, to find the optimal settings of a transformation and learner.

\item \begin{com}
Page 11 Figure 8. The authors didn’t explain the results from PitsA. In this case, both DODGE and FFT are worse than LDADE SVM.
\end{com}

Recall that these are results from multiple trials so we should look at the distributions (using statistics)
and not point values. As mentioned in the text, 
LDADE SVM do not statistically win against FFT or \IT*.

\item \begin{com}
Figure 8. This paper divides the treatments of Figure 8 into several groups. But it is hard to read the improvements between groups. 
\end{com}

You are correct-- there was no value added in that separation into different groups. We have removed that
text.

% No learner wins all the time on all data (see Wolpert's no free lunch theories).
% In the particular case of that result, {\IT*} loses to LDA-FFT. That is to 

% In figure~\ref{fig:text}, \IT* wins on an average of about 20\%   against LDADE~\cite{agrawal2018wrong} and LDA-GA~\cite{Panichella:2013}, the 2 state-of-the-art hyperparameter optimizers. These are the major 2 groups in the figure, which are actually tuning a transformation algorithm (LDA) combined with different learners such as FFT and SVM. 

\item \begin{com}
The author describes the external validity. I am wondering if there is any internal validity in this paper. If it has, please give the details.
\end{com}

Yes we have added some other threats to validity. The internal validity is addressed in the construct validity of Section~\ref{sect:threats}.

\item \begin{com}
(typos listed)
\end{com}

Fixed! Thanks for finding these!

\ee

==> reply2.tex <==
\newpage
  \pagenumbering{roman}
\setcounter{page}{1}

\newenvironment{com}{\color{blue}\begin{itshape}}{\end{itshape}\vspace{1ex}}

\section*{Response to Reviewers}

Please see our replies to reviewer comments, below. Note that anything in \begin{com}
blue
\end{com} is from the reviewers. Our replies are in  \textbf{black} text.

\subsection*{Associate Editor}
\label{sec:AE}

\begin{com}
Comments to the Author:
Thank you for your revision. The reviewers are largely satisfied, but some lingering concerns remain. Once you make this minor revision, I will review the changes myself, and decide if the manuscript is yet ready for acceptance.
\end{com}

We would like to thank all our reviewers for their support. Please see our responses to their reviews below.

\subsection*{Reviewer 1}
\label{sec:Reviewer1}
\renewcommand*{\theenumi}{1.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}

\be 
\item \begin{com}

Thanks authors for carefully addressing my comments. After my careful read on this revision and responses, this is an excellent work and I'm happy to recommend acceptance. 

\end{com}

Thank you very much for your careful review
and all your great advice!  Much appreciated!

We are very excited
about this result. We think it changes the nature
of hyperparameter optimization in the field of SE--
makes it something that is now so easy that everyone
can do it, routinely.

\item \begin{com}

Please include the response in the paper where appropriate (e.g., 1.11).

In addition to \cite{tantithamthavorn2016automated}, please include \url{https://ieeexplore.ieee.org/document/8263202} as well.
\end{com}

Added! Now, throughout the paper, every place we reference ~\cite{tantithamthavorn2016automated} we also reference~\cite{8263202}

\item \begin{com}

1.1 - 1.6) Thanks

1.7) Actually, Accuracy of predictions means precision, recall, F-measure, d2h. As you argued that DODGE gets higher performance with faster termination. I'm fine with that.

1.8 - 1.10) Thanks

1.12 - 1.21) Thanks

1.11) Please include the justification in the paper as well. 
\end{com}

We have done so... please see the new caption of Table~6.

\ee 



\subsection*{Reviewer 2}
\label{sec:Reviewer2}
\renewcommand*{\theenumi}{2.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}

\be 
\item \begin{com}

I thank the authors for considering my comments. The revised structure of the article is better and the clarifications to support the understanding of DODGE and FFTrees are valuable. I am particularly happy to see the new related work section as it clearly positions the DODGE contribution and outlines future work. To help other researchers explore DODGE, perhaps a next step could be to organize a tutorial at some major conference?

\end{com}

Thank you very much for your careful review
and all your great advice!  Much appreciated!

Regarding your suggestion of a tutorial... that is a very interesting idea. Perhaps we could team up with
some of the other people doing SE
hyperparameter optimization and make it a bit
of a festival.  

\item \begin{com}

The new abstract is much better, but I still think the authors should reconsider the use of parentheses. If text is peripheral enough to end up within parentheses, then it should perhaps not be in the abstract at all? In the revised abstract, 30\% of the words are still within parentheses.

\end{com}

This is very good advice. We have removed
all parentheses from the abstract.

\begin{com}

My other comments have all been properly addressed, and my points below are all related to language/typos.

[list of typos]

\end{com}

Thank you for your careful proofread and
that list of typos. All fixed now.

% \begin{com}
% Missing whitespace after the author Di Chen and after (xshen5@ncsu.edu) on the first page
% Page 3:22 – 1,600 exabytes
% Page 4:5 – “reduced” (consistent verb tense)
% Fig. 4 – nouns in plural? billions of combinations, ranges of attributes, for categorical values
% Page 10:37 - learners
% Page 10:52 – bias was a required and needed
% Page 11:3 – there is no closing parenthesis
% Page 11:38 – missing thousands separator
% \end{com}

\ee

\subsection*{Reviewer 3}
\label{sec:Reviewer3}
\renewcommand*{\theenumi}{3.\arabic{enumi}}
\renewcommand*{\theenumii}{\theenumi.\arabic{enumii}}

\be 
\item \begin{com}

I am satisfied with the work of the authors to improve their manuscript.  They managed to address each of my comments in the best possible way.

\end{com}

Thank you very much for your careful review
and all your great advice!  Much appreciated!

\item \begin{com}
There are, however, some minor changes that have to be addressed.

1.My first concern is about the generalizability of DODGE. The author describes DODGE as a hyper-parameter tuning framework independent of the learning algorithm it was applied on. However, the learners which DODGE chose are most elementary learning algorithms with a small number of hyper-parameters. It is worth studying the effect of DODGE on more complex machine learning algorithms like neural networks.  

\end{com}

You raise an important point. We have added
text on this matter in our threats to validity section
(under {\bf Learner Bias}):
\begin{quote}
{\em One important class of learners not studied 
here are those that use numerous
hyperparameters. 
All the learners explored here by DODGE  have less than
dozen hyperparameters.
In the future, it would be worth  
studying the value of DODGE on more complex  machine  learning  algorithms  such as  neural  networks. }
\end{quote}


\item \begin{com}
2.There is a concern on the figure 2, which task is used to evaluate the computation cost of different methods? And the authors mentioned that DODGE is faster than others, what does “faster” mean (less cost or less time)?
\end{com}

In this figure, it represents the number of evaluations taken by each method to identify an optimal model. Cost and Time can be interchangeable terms, here, we say reduction in time by finding less number of evaluations. But at the same time, we would require lesser costlier resources like CPU and GPU since number of evaluations taken are less. 

\item \begin{com}
3.For the comparison between DODGE and other tuning techniques, did you keep the learners of those baselines same as DODGE?  
\end{com}

We used the same learners for DODGE and other tuning techniques as well as, they appeared in prior
state of the art papers. We   would say that
this is an appropriate, even respectful,
way to comapre prior work with the results of this paper

\item \begin{com}

4.RQ3 aims to study whether DODGE is useful for tasks other than defect prediction, but the authors only use one task (text mining) to prove their hypothesis. Maybe the RQ should be changed to “is DODGE useful for software text mining?”
\end{com}

We will take the advice of the associate editor
on this point. As we read this comment, this seems like an optional point for you.  Our view is that we can leave it as is, (but will certainly
work as directed on this point).

\item \begin{com}

5.The reason why DODGE perform worse than all baselines in several datasets are not well-explained. Particularly, on the text mining task, since the size of pitsB is larger than other datasets, I believe this issue is worth further studying and may lead to some weaknesses of DODGE.
\end{com}

This is a very important point. We agree that this
matter is worth further exploring. FYI- we have some preliminary results on this issue: it turns out
that the size of the target class is an important factor.
Specifically, 
when the target class becomes less frequent, then:
it is harder to find the target; and
the larger the observed $\epsilon$
in the results;
and the  greater the number of redundant tunings; 
and the more likely that DODGE will work.

That said, at this time, those new results need some further work and we would be nervous placing them into this article.

\item \begin{com}
6.Page 1. Table 1 was explained twice. The author should merge those two descriptions.
\end{com}

You are right. We have modified the second explanation to point out an important aspect of that table:
\begin{quote}
{\em \tbl{options} is  a partial
list of some of the  tunings that might be explored. 
Even this incomplete sample includes billions of configuration options.}
\end{quote}

\item \begin{com}
7.Page 6. Figure 3 is redundant. I believe these results were already shown in [16]?
\end{com}

Your make a good point. To address this issue,
just so that the reader knows that the result
of this one table is {\bf NOT} new work,
we have added "From~\cite{chen2018applications}." in the caption of that figure.

\ee

==> temp_old.tex <==

\subsubsection{How to Study Defect Prediction?}


cohen= 4 for fig8 d2h



This section shows the FFtree results that lead to 
the design of \IT*. DODGE. After that, 
\section{Accidental Simplification with FFTtrees}
\subsection{ Simplification is Possible?}
AI researchers have repeatedly concluded that a small number of {\em key} variables determine the behavior of the rest of the system. Keys have been discovered and rediscovered   many times and given different names,
including feature subset selection~\cite{kohavi1997wrappers}, narrows~\cite{michalski2013machine}, master variables~\ctie{Crawford1994ExperimentalRO},  and back doors~\cite{Williams:2003}.

We mention this since the  problem of mining data  with keys reduces to just the mining the key variables.
For many years, we have been acc


For over a  decade now, we have been documenting examples were solutions to SE analytics problems were surprisingly simple (but until {\IT*}, we had no explanation for that phenomenon nor a method to exploit that simpilicity).
For example, when optimizing requirements engineering, we have often found that most requirements are dependent on just a few {\em key} choices. We have exploited this effect 
to simpigy reasoning about requirements engineering models. For example, fat NASA'sJey ropulsion aroty, we dted a decison procesdure impmeeted as a genatic algorithm. While the GA offered decision of 90 decisions, we found 30 keys which (once decided) controlled the rest. 

 

\subsection{Exploiting $\mathcal{E}$  } 
 Many methods have been proposed  to reduce the above uncertainties.
 For example, in our research we have explored
 feature selection to remove spurious outliers~\cite{menzies2007data}, application of
 background knowledge to constrain model generation~\cite{fenton2012risk}, and optimizers to tune model parameters to reduce uncertainty~\cite{Agrawal18stab}.
 Despite all that work, some degree of uncertainty in the results
 from software analytics persists (for a detailed analysis on this point, see~\cite{menzies2012special}).
 We conjecture that, for all     reasons listed in the last section,
uncertainty is an inherent property of software quality prediction. If so, the question becomes, ``what to do with that uncertainty?''.
 


 The starting point for this article was the following speculation:
 \textbf{\em{ Instead of striving to make $\mathcal{E}=0$, use $\mathcal{E}>0$ as a method for simplifying software quality predictors}}. For example,
Deb's principle of $\mathcal{E}$-dominance~\cite{deb2005evaluating} 
states that if there exists
some  $\mathcal{E}$ value below
which is useless or impossible to distinguish results, then
it is superfluous to explore anything less than $\mathcal{E}$.

Note that $\mathcal{E}$ effectively clusters the space of possible results.
For example, consider the result space defined by recall $r$ and false alarms $f$.
Both these measures have the  range \mbox{$0 \le r \le 1$} and
 \mbox{$0 \le f \le 1$}.
 Large values of $\mathcal{E}$ divide the results
 into just a few regions. For example, when 
 \mbox{ $\mathcal{E}=0.2$}, then the results space of possible recalls and false alarms divides into the 5*5 grid of \fig{resultspace}.  Most learners avoid the red regions (where recall is worse than false alarms) and the gray region (called the no-information region).
 Hence, 
  when \mbox{$\mathcal{E}=0.2$}, learners produce results
  that uusally fall into  a small number of regions (just the ten
  green squares of \fig{resultspace}).  
 
 Now consider the implications of large $\mathcal{E}$ 
 for exploring hyperparameter optimization. Recall that such optimizers find a few useful options by exploring
 a very large number of options. Given a results space like
 \fig{resultspace}, many of those options will fall into the same regions. If we mark which options generate results that fall within $\mathcal{E}$ of other results,
 then we strive to avoid those options in the future,
 then theoretically we might be able to search across  \fig{resultspace}, very quickly.


\subsection{{\IT*}}

A sketch of the {\IT*} algorithm was offered in the introduction.
This section offers other details about {\IT*}.

{\IT*} inputs a tree of options $o_1..o_m$ (like \tbl{options}) as well as some constraints describing what sets of options are illegal (for example, see the last line of that figure).
Some options contain a range (e.g. {\em Binarizer}'s threshold ranges from 0 to 100). Each such option  gets 100 sub-trees that divide
its range into 100 sub-ranges.

{\IT*} then attaches a counter $c_i$ to each leaf  and each node
in the tree.  If ever a leaf counter is incremented or decremented by 1,
then all the counts in the branch leading to that leaf are incremeneted or decremented by the same amount.  

The option tree in {\IT*} is processed by two sub-routines: {\em Generate} and {\em ReCount}.
\bi
\item {\em Generate} is called prior to running a learner to generate some tuning options $T$. {\em Generate}
is a recursive descent down two trees: one for the learners and one for the data pre-processors. At each level, {\em Guess} will recurse into the subtree with highest counter value. 
\item {\em ReCount}  is called after running a learner (using options $T$) and its performance score is available. If that score is within $\mathcal{E}$ of a prior score,
then {\em ReCount} will minus one from all the options $o \in T$.
Else, it will add one.
\ei
XXXX note that next Guess will recountxxx

. For example, in \tbl{options}, The rest of this article explores this theoretical prediction using {\IT*}, an algorithm that implements the procedure
of the last paragraph.
 
 %XXXX why do not reported before. culture that rewards increasing complexity. all too tempting to solve problems with long runtime, just by applying more hardware
 \section{Methods}
 \subsection{Problem Domains}
 This article tests {\IT*} in the four domains listed in the introduction. These domains use defect prediction,
 
  

\subsection{{\IT*}: Exploiting Large $\mathcal{E}$} 
   


We can exploit this effect as follows. Suppose we 

%  \begin{table*}[!t]
%      \caption{Classifiers used in this study. Rankings from Ghotra et al.~\cite{ghotra2015revisiting}.}
%      \label{tbl:ourlearners}
%      \footnotesize
%      \begin{tabular}{l|l|p{4.85in}}
%      \hline
%     \rowcolor{lightgray} 
%     {\bf RANK} & {\bf LEARNER} & {\bf NOTES}\\\hline
%      1 (best) & Random Forest~(RF) & 
%      Generate conclusions using multiple entropy-based decision trees.\\\cline{2-3}
%      &  Logistic Regression~(SL) & Map the output of a regression into $0\le n \le 1$; thus enabling using regression for classification (e.g., defective if $n>0.5$).\\\hline
%      2 & K Nearest Neighbors~(KNN) &  Classify a new instance by finding ``k'' examples of similar instances.
%      Ghortra et al. suggested
%      $K=8$.\\\cline{2-3}
%      &  \multirow{2}{*}{Naive Bayes~(NB)} &  Classify a new instance by (a)~collecting mean and standard deviations of attributes in old instances of  different classes; (b)~return the class whose attributes are statistically most similar to the new instance.\\\hline
%      3 & Decision Trees~(DT) & Recursively
%      divide data by selecting attribute splits
%      that reduce the entropy of the class distribution.\\\cline{2-3}
%      & Expectation Maximization (EM) & This clustering algorithm uses iterative sampling and repair to derive a parametric expression for each class. \\\hline
    
%      4 (worst) & Support Vector Machines~(SMO) &
%      Map the raw data into a higher-dimensional space where it is easier to distinguish the examples.
%      \\\hline
%      \end{tabular}
%      \vspace{-0.2cm}
%  \end{table*}
% Another reason to study simplification is that studies can reveal the underlying nature of seemingly
% complex problems.
% In terms of core science, we argue that the better we understand
% something, the better we can match tools to SE. Tools
% which are poorly matched to task are usually complex and/or
% slow to execute. DART seems a better match for the tasks explored
% in this article since it is neither complex nor slow. Hence,
% we argue that DART is interesting in terms of its core scientific
% contribution to SE quality prediction.







 \begin{figure*}

 \begin{tabular}{|p{.48\linewidth}|p{.48\linewidth}|}\hline 
{\bf Software Defect Prediction}
 \bi
 \item
Software developers are smart, but sometimes make mistakes. Hence, it is essential to test software before the deployment ~\cite{orso2014software,barr2015oracle,yoo2012regression, myers2011art}. 
\item
 Software quality assurance budgets are finite while assessment effectiveness increases exponentially with assessment effort~\cite{fu2016tuning}. Therefore,  standard practice is to apply the best available methods on code sections that seem most critical and bug-prone.
\item
Software bugs are not evenly distributed across the project~\cite{hamill2009common,koru2009investigation, ostrand2004bugs,misirli2011ai}.  Hence, 
a useful way to perform software testing is to allocate most assessment budgets to
the more defect-prone parts in software projects.   
\item
Software defect predictors are never 100\% correct. But
they can be used to suggest where to focus more expensive methods. 
\item
Software defect predictors have been proven useful in many industrial settings. 
When Misirli et al.~\cite{misirli2011ai} built a  defect prediction model  for a telecommunications company, those  models
could  predict 87 percent of code defects.
Those models also decreased inspection efforts by 72 percent, and hence reduce post-release defects by 44 percent. Also, when Kim et al.~\cite{kim2015remi} applied defect prediction model, REMI, to API
development process at Samsung Electronics, they found they could
predicted the bug-prone APIs with reasonable accuracy~(0.68 F1 score)
and reduced the resources required for executing test cases.
\item
Software defect predictors not only save labor compared with traditional manual methods, but they are also competitive with certain automatic methods.  
A recent study at ICSE'14, Rahman et al. ~\cite{rahman2014comparing} compared (a) static code analysis tools FindBugs, Jlint, and PMD and (b) static code defect predictors (which they called ``statistical defect prediction'') built using logistic  regression.
They found no significant differences in the cost-effectiveness of these approaches.  
\item
Given this equivalence, it is significant to
note that static code defect prediction can be quickly adapted to new languages by building lightweight parsers that find in-
formation  like  Table ~\ref{tbl:ck}.  The same is not true for static code analyzers - these need extensive modification before they can be used in new languages.
\ei
&
{\bf Software bug report text mining }

\end{tabular}
\end{figure*}

